Domain Generalisation for Apparent Emotional Facial Expression Recognition across Age-Groups

Apparent emotional facial expression recognition has attracted a lot of research attention recently. However, the majority of approaches ignore age differences and train a generic model for all ages. In this work, we study the effect of using different age-groups for training apparent emotional facial expression recognition models. To this end, we study Domain Generalisation in the context of apparent emotional facial expression recognition from facial imagery across different age groups. We first compare several domain generalisation algorithms on the basis of out-of-domain-generalisation, and observe that the Class-Conditional Domain-Adversarial Neural Networks (CDANN) algorithm has the best performance. We then study the effect of variety and number of age-groups used during training on generalisation to unseen age-groups and observe that an increase in the number of training age-groups tends to increase the apparent emotional facial expression recognition performance on unseen age-groups. We also show that exclusion of an age-group during training tends to affect more the performance of the neighbouring age groups.

==> sections/other_tables.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{llrrrrrr}
%     \toprule
%         &          &  g2a0-18 &  g2a60-85 &  g2a50-60 &  g2a40-50 &  g2a30-40 &  g2a18-30 \\
%     \midrule
%     0   & Arousal\_CCC &    0.640 &     0.529 &       NaN &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.858 &     0.789 &       NaN &       NaN &       NaN &       NaN \\
%         & nLoss &    0.794 &     1.203 &       NaN &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.805 &     0.695 &       NaN &       NaN &       NaN &       NaN \\
%     1   & Arousal\_CCC &    0.638 &       NaN &     0.573 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.860 &       NaN &     0.817 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.807 &       NaN &     1.118 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.803 &       NaN &     0.716 &       NaN &       NaN &       NaN \\
%     2   & Arousal\_CCC &    0.632 &       NaN &       NaN &     0.615 &       NaN &       NaN \\
%         & Valence\_CCC &    0.856 &       NaN &       NaN &     0.826 &       NaN &       NaN \\
%         & nLoss &    0.797 &       NaN &       NaN &     0.983 &       NaN &       NaN \\
%         & Accuracy &    0.810 &       NaN &       NaN &     0.751 &       NaN &       NaN \\
%     3   & Arousal\_CCC &    0.642 &       NaN &       NaN &       NaN &     0.620 &       NaN \\
%         & Valence\_CCC &    0.861 &       NaN &       NaN &       NaN &     0.823 &       NaN \\
%         & nLoss &    0.789 &       NaN &       NaN &       NaN &     0.947 &       NaN \\
%         & Accuracy &    0.809 &       NaN &       NaN &       NaN &     0.767 &       NaN \\
%     4   & Arousal\_CCC &    0.585 &       NaN &       NaN &       NaN &       NaN &     0.576 \\
%         & Valence\_CCC &    0.843 &       NaN &       NaN &       NaN &       NaN &     0.817 \\
%         & nLoss &    0.889 &       NaN &       NaN &       NaN &       NaN &     0.979 \\
%         & Accuracy &    0.788 &       NaN &       NaN &       NaN &       NaN &     0.768 \\
%     101 & Arousal\_CCC &    0.653 &     0.496 &     0.565 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.866 &     0.772 &     0.816 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.758 &     1.285 &     1.114 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.814 &     0.675 &     0.709 &       NaN &       NaN &       NaN \\
%     102 & Arousal\_CCC &    0.634 &     0.491 &       NaN &     0.589 &       NaN &       NaN \\
%         & Valence\_CCC &    0.858 &     0.765 &       NaN &     0.818 &       NaN &       NaN \\
%         & nLoss &    0.835 &     1.394 &       NaN &     1.101 &       NaN &       NaN \\
%         & Accuracy &    0.803 &     0.664 &       NaN &     0.735 &       NaN &       NaN \\
%     103 & Arousal\_CCC &    0.624 &     0.491 &       NaN &       NaN &     0.601 &       NaN \\
%         & Valence\_CCC &    0.859 &     0.787 &       NaN &       NaN &     0.821 &       NaN \\
%         & nLoss &    0.822 &     1.291 &       NaN &       NaN &     0.991 &       NaN \\
%         & Accuracy &    0.808 &     0.679 &       NaN &       NaN &     0.756 &       NaN \\
%     112 & Arousal\_CCC &    0.642 &       NaN &     0.563 &     0.604 &       NaN &       NaN \\
%         & Valence\_CCC &    0.862 &       NaN &     0.813 &     0.823 &       NaN &       NaN \\
%         & nLoss &    0.788 &       NaN &     1.150 &     1.033 &       NaN &       NaN \\
%         & Accuracy &    0.812 &       NaN &     0.710 &     0.746 &       NaN &       NaN \\
%     113 & Arousal\_CCC &    0.617 &       NaN &     0.541 &       NaN &     0.596 &       NaN \\
%         & Valence\_CCC &    0.854 &       NaN &     0.803 &       NaN &     0.812 &       NaN \\
%         & nLoss &    0.897 &       NaN &     1.329 &       NaN &     1.094 &       NaN \\
%         & Accuracy &    0.800 &       NaN &     0.695 &       NaN &     0.753 &       NaN \\
%     \bottomrule
%     \end{tabular}
%     \caption{CDANN}
%     \label{tab:my_label}
% \end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{llrrrrrr}
%     \toprule
%         &          &  g2a0-18 &  g2a60-85 &  g2a50-60 &  g2a40-50 &  g2a30-40 &  g2a18-30 \\
%     \midrule
%     0   & Arousal\_CCC &    0.601 &     0.491 &       NaN &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.851 &     0.770 &       NaN &       NaN &       NaN &       NaN \\
%         & nLoss &    0.888 &     1.407 &       NaN &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.786 &     0.661 &       NaN &       NaN &       NaN &       NaN \\
%     1   & Arousal\_CCC &    0.506 &       NaN &     0.415 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.811 &       NaN &     0.743 &       NaN &       NaN &       NaN \\
%         & nLoss &    1.171 &       NaN &     1.756 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.725 &       NaN &     0.596 &       NaN &       NaN &       NaN \\
%     2   & Arousal\_CCC &    0.597 &       NaN &       NaN &     0.573 &       NaN &       NaN \\
%         & Valence\_CCC &    0.849 &       NaN &       NaN &     0.810 &       NaN &       NaN \\
%         & nLoss &    0.920 &       NaN &       NaN &     1.183 &       NaN &       NaN \\
%         & Accuracy &    0.786 &       NaN &       NaN &     0.725 &       NaN &       NaN \\
%     3   & Arousal\_CCC &    0.604 &       NaN &       NaN &       NaN &     0.592 &       NaN \\
%         & Valence\_CCC &    0.827 &       NaN &       NaN &       NaN &     0.798 &       NaN \\
%         & nLoss &    0.866 &       NaN &       NaN &       NaN &     1.010 &       NaN \\
%         & Accuracy &    0.797 &       NaN &       NaN &       NaN &     0.754 &       NaN \\
%     4   & Arousal\_CCC &    0.517 &       NaN &       NaN &       NaN &       NaN &     0.466 \\
%         & Valence\_CCC &    0.794 &       NaN &       NaN &       NaN &       NaN &     0.777 \\
%         & nLoss &    1.007 &       NaN &       NaN &       NaN &       NaN &     1.150 \\
%         & Accuracy &    0.773 &       NaN &       NaN &       NaN &       NaN &     0.734 \\
%     101 & Arousal\_CCC &    0.623 &     0.481 &     0.544 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.855 &     0.750 &     0.801 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.864 &     1.351 &     1.208 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.810 &     0.675 &     0.702 &       NaN &       NaN &       NaN \\
%     102 & Arousal\_CCC &    0.613 &     0.496 &       NaN &     0.589 &       NaN &       NaN \\
%         & Valence\_CCC &    0.853 &     0.771 &       NaN &     0.818 &       NaN &       NaN \\
%         & nLoss &    0.832 &     1.296 &       NaN &     1.048 &       NaN &       NaN \\
%         & Accuracy &    0.802 &     0.679 &       NaN &     0.744 &       NaN &       NaN \\
%     103 & Arousal\_CCC &    0.601 &     0.471 &       NaN &       NaN &     0.576 &       NaN \\
%         & Valence\_CCC &    0.851 &     0.761 &       NaN &       NaN &     0.804 &       NaN \\
%         & nLoss &    0.905 &     1.464 &       NaN &       NaN &     1.110 &       NaN \\
%         & Accuracy &    0.797 &     0.660 &       NaN &       NaN &     0.743 &       NaN \\
%     112 & Arousal\_CCC &    0.565 &       NaN &     0.515 &     0.555 &       NaN &       NaN \\
%         & Valence\_CCC &    0.843 &       NaN &     0.803 &     0.813 &       NaN &       NaN \\
%         & nLoss &    0.882 &       NaN &     1.194 &     1.080 &       NaN &       NaN \\
%         & Accuracy &    0.795 &       NaN &     0.696 &     0.732 &       NaN &       NaN \\
%     113 & Arousal\_CCC &    0.620 &       NaN &     0.549 &       NaN &     0.597 &       NaN \\
%         & Valence\_CCC &    0.847 &       NaN &     0.806 &       NaN &     0.809 &       NaN \\
%         & nLoss &    0.910 &       NaN &     1.211 &       NaN &     1.077 &       NaN \\
%         & Accuracy &    0.805 &       NaN &     0.703 &       NaN &     0.750 &       NaN \\
%     \bottomrule
%     \end{tabular}
%     \caption{ERM}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{llrrrrrr}
%     \toprule
%         &          &  g2a0-18 &  g2a60-85 &  g2a50-60 &  g2a40-50 &  g2a30-40 &  g2a18-30 \\
%     \midrule
%     0   & Arousal\_CCC &    0.615 &     0.500 &       NaN &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.853 &     0.783 &       NaN &       NaN &       NaN &       NaN \\
%         & nLoss &    0.848 &     1.273 &       NaN &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.798 &     0.678 &       NaN &       NaN &       NaN &       NaN \\
%     1   & Arousal\_CCC &    0.622 &       NaN &     0.553 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.846 &       NaN &     0.802 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.891 &       NaN &     1.193 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.809 &       NaN &     0.710 &       NaN &       NaN &       NaN \\
%     2   & Arousal\_CCC &    0.587 &       NaN &       NaN &     0.558 &       NaN &       NaN \\
%         & Valence\_CCC &    0.847 &       NaN &       NaN &     0.803 &       NaN &       NaN \\
%         & nLoss &    0.940 &       NaN &       NaN &     1.184 &       NaN &       NaN \\
%         & Accuracy &    0.788 &       NaN &       NaN &     0.721 &       NaN &       NaN \\
%     3   & Arousal\_CCC &    0.564 &       NaN &       NaN &       NaN &     0.533 &       NaN \\
%         & Valence\_CCC &    0.835 &       NaN &       NaN &       NaN &     0.787 &       NaN \\
%         & nLoss &    1.023 &       NaN &       NaN &       NaN &     1.253 &       NaN \\
%         & Accuracy &    0.786 &       NaN &       NaN &       NaN &     0.725 &       NaN \\
%     4   & Arousal\_CCC &    0.573 &       NaN &       NaN &       NaN &       NaN &     0.568 \\
%         & Valence\_CCC &    0.829 &       NaN &       NaN &       NaN &       NaN &     0.806 \\
%         & nLoss &    0.919 &       NaN &       NaN &       NaN &       NaN &     0.999 \\
%         & Accuracy &    0.783 &       NaN &       NaN &       NaN &       NaN &     0.763 \\
%     101 & Arousal\_CCC &    0.622 &     0.483 &     0.549 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.857 &     0.744 &     0.803 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.830 &     1.383 &     1.188 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.800 &     0.652 &     0.695 &       NaN &       NaN &       NaN \\
%     102 & Arousal\_CCC &    0.600 &     0.443 &       NaN &     0.559 &       NaN &       NaN \\
%         & Valence\_CCC &    0.848 &     0.748 &       NaN &     0.808 &       NaN &       NaN \\
%         & nLoss &    0.879 &     1.435 &       NaN &     1.126 &       NaN &       NaN \\
%         & Accuracy &    0.799 &     0.661 &       NaN &     0.733 &       NaN &       NaN \\
%     103 & Arousal\_CCC &    0.582 &     0.419 &       NaN &       NaN &     0.538 &       NaN \\
%         & Valence\_CCC &    0.842 &     0.741 &       NaN &       NaN &     0.796 &       NaN \\
%         & nLoss &    1.021 &     1.767 &       NaN &       NaN &     1.262 &       NaN \\
%         & Accuracy &    0.781 &     0.634 &       NaN &       NaN &     0.726 &       NaN \\
%     112 & Arousal\_CCC &    0.597 &       NaN &     0.530 &     0.575 &       NaN &       NaN \\
%         & Valence\_CCC &    0.829 &       NaN &     0.788 &     0.803 &       NaN &       NaN \\
%         & nLoss &    0.878 &       NaN &     1.190 &     1.072 &       NaN &       NaN \\
%         & Accuracy &    0.793 &       NaN &     0.694 &     0.733 &       NaN &       NaN \\
%     113 & Arousal\_CCC &    0.587 &       NaN &     0.536 &       NaN &     0.580 &       NaN \\
%         & Valence\_CCC &    0.829 &       NaN &     0.797 &       NaN &     0.801 &       NaN \\
%         & nLoss &    0.912 &       NaN &     1.194 &       NaN &     1.058 &       NaN \\
%         & Accuracy &    0.802 &       NaN &     0.702 &       NaN &     0.750 &       NaN \\
%     \bottomrule
%     \end{tabular}
%     \caption{MMD}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{llrrrrrr}
%     \toprule
%         &          &  g2a0-18 &  g2a60-85 &  g2a50-60 &  g2a40-50 &  g2a30-40 &  g2a18-30 \\
%     \midrule
%     0   & Arousal\_CCC &    0.581 &     0.454 &       NaN &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.846 &     0.759 &       NaN &       NaN &       NaN &       NaN \\
%         & nLoss &    0.881 &     1.355 &       NaN &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.791 &     0.663 &       NaN &       NaN &       NaN &       NaN \\
%     1   & Arousal\_CCC &    0.586 &       NaN &     0.536 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.843 &       NaN &     0.801 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.890 &       NaN &     1.170 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.788 &       NaN &     0.702 &       NaN &       NaN &       NaN \\
%     2   & Arousal\_CCC &    0.615 &       NaN &       NaN &     0.598 &       NaN &       NaN \\
%         & Valence\_CCC &    0.850 &       NaN &       NaN &     0.819 &       NaN &       NaN \\
%         & nLoss &    0.833 &       NaN &       NaN &     1.035 &       NaN &       NaN \\
%         & Accuracy &    0.800 &       NaN &       NaN &     0.743 &       NaN &       NaN \\
%     3   & Arousal\_CCC &    0.570 &       NaN &       NaN &       NaN &     0.581 &       NaN \\
%         & Valence\_CCC &    0.827 &       NaN &       NaN &       NaN &     0.795 &       NaN \\
%         & nLoss &    0.916 &       NaN &       NaN &       NaN &     1.045 &       NaN \\
%         & Accuracy &    0.780 &       NaN &       NaN &       NaN &     0.744 &       NaN \\
%     4   & Arousal\_CCC &    0.571 &       NaN &       NaN &       NaN &       NaN &     0.563 \\
%         & Valence\_CCC &    0.831 &       NaN &       NaN &       NaN &       NaN &     0.803 \\
%         & nLoss &    0.934 &       NaN &       NaN &       NaN &       NaN &     1.032 \\
%         & Accuracy &    0.788 &       NaN &       NaN &       NaN &       NaN &     0.761 \\
%     101 & Arousal\_CCC &    0.625 &     0.477 &     0.547 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.859 &     0.753 &     0.804 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.821 &     1.407 &     1.205 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.802 &     0.655 &     0.692 &       NaN &       NaN &       NaN \\
%     102 & Arousal\_CCC &    0.622 &     0.523 &       NaN &     0.596 &       NaN &       NaN \\
%         & Valence\_CCC &    0.853 &     0.775 &       NaN &     0.819 &       NaN &       NaN \\
%         & nLoss &    0.826 &     1.258 &       NaN &     1.037 &       NaN &       NaN \\
%         & Accuracy &    0.803 &     0.678 &       NaN &     0.740 &       NaN &       NaN \\
%     103 & Arousal\_CCC &    0.610 &     0.517 &       NaN &       NaN &     0.597 &       NaN \\
%         & Valence\_CCC &    0.845 &     0.767 &       NaN &       NaN &     0.813 &       NaN \\
%         & nLoss &    0.856 &     1.297 &       NaN &       NaN &     1.012 &       NaN \\
%         & Accuracy &    0.799 &     0.676 &       NaN &       NaN &     0.752 &       NaN \\
%     112 & Arousal\_CCC &    0.606 &       NaN &     0.526 &     0.579 &       NaN &       NaN \\
%         & Valence\_CCC &    0.843 &       NaN &     0.800 &     0.808 &       NaN &       NaN \\
%         & nLoss &    0.878 &       NaN &     1.271 &     1.130 &       NaN &       NaN \\
%         & Accuracy &    0.796 &       NaN &     0.690 &     0.728 &       NaN &       NaN \\
%     113 & Arousal\_CCC &    0.569 &       NaN &     0.537 &       NaN &     0.576 &       NaN \\
%         & Valence\_CCC &    0.841 &       NaN &     0.798 &       NaN &     0.802 &       NaN \\
%         & nLoss &    0.897 &       NaN &     1.191 &       NaN &     1.042 &       NaN \\
%         & Accuracy &    0.786 &       NaN &     0.694 &       NaN &     0.746 &       NaN \\
%     \bottomrule
%     \end{tabular}
%     \caption{MLDG}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{llrrrrrr}
%     \toprule
%         &          &  g2a0-18 &  g2a60-85 &  g2a50-60 &  g2a40-50 &  g2a30-40 &  g2a18-30 \\
%     \midrule
%     0   & Arousal\_CCC &    0.602 &     0.492 &       NaN &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.846 &     0.765 &       NaN &       NaN &       NaN &       NaN \\
%         & nLoss &    0.858 &     1.258 &       NaN &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.799 &     0.687 &       NaN &       NaN &       NaN &       NaN \\
%     1   & Arousal\_CCC &    0.622 &       NaN &     0.569 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.853 &       NaN &     0.815 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.834 &       NaN &     1.119 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.806 &       NaN &     0.714 &       NaN &       NaN &       NaN \\
%     2   & Arousal\_CCC &    0.630 &       NaN &       NaN &     0.604 &       NaN &       NaN \\
%         & Valence\_CCC &    0.837 &       NaN &       NaN &     0.811 &       NaN &       NaN \\
%         & nLoss &    0.863 &       NaN &       NaN &     1.048 &       NaN &       NaN \\
%         & Accuracy &    0.805 &       NaN &       NaN &     0.744 &       NaN &       NaN \\
%     3   & Arousal\_CCC &    0.594 &       NaN &       NaN &       NaN &     0.566 &       NaN \\
%         & Valence\_CCC &    0.836 &       NaN &       NaN &       NaN &     0.798 &       NaN \\
%         & nLoss &    0.918 &       NaN &       NaN &       NaN &     1.105 &       NaN \\
%         & Accuracy &    0.794 &       NaN &       NaN &       NaN &     0.744 &       NaN \\
%     4   & Arousal\_CCC &    0.565 &       NaN &       NaN &       NaN &       NaN &     0.561 \\
%         & Valence\_CCC &    0.828 &       NaN &       NaN &       NaN &       NaN &     0.804 \\
%         & nLoss &    0.961 &       NaN &       NaN &       NaN &       NaN &     1.037 \\
%         & Accuracy &    0.779 &       NaN &       NaN &       NaN &       NaN &     0.762 \\
%     101 & Arousal\_CCC &    0.645 &     0.508 &     0.564 &       NaN &       NaN &       NaN \\
%         & Valence\_CCC &    0.851 &     0.752 &     0.802 &       NaN &       NaN &       NaN \\
%         & nLoss &    0.828 &     1.291 &     1.155 &       NaN &       NaN &       NaN \\
%         & Accuracy &    0.815 &     0.683 &     0.711 &       NaN &       NaN &       NaN \\
%     102 & Arousal\_CCC &    0.614 &     0.519 &       NaN &     0.603 &       NaN &       NaN \\
%         & Valence\_CCC &    0.849 &     0.779 &       NaN &     0.813 &       NaN &       NaN \\
%         & nLoss &    0.841 &     1.228 &       NaN &     1.031 &       NaN &       NaN \\
%         & Accuracy &    0.804 &     0.689 &       NaN &     0.745 &       NaN &       NaN \\
%     103 & Arousal\_CCC &    0.601 &     0.529 &       NaN &       NaN &     0.604 &       NaN \\
%         & Valence\_CCC &    0.842 &     0.781 &       NaN &       NaN &     0.810 &       NaN \\
%         & nLoss &    0.878 &     1.218 &       NaN &       NaN &     1.019 &       NaN \\
%         & Accuracy &    0.797 &     0.696 &       NaN &       NaN &     0.755 &       NaN \\
%     112 & Arousal\_CCC &    0.610 &       NaN &     0.567 &     0.601 &       NaN &       NaN \\
%         & Valence\_CCC &    0.849 &       NaN &     0.808 &     0.818 &       NaN &       NaN \\
%         & nLoss &    0.838 &       NaN &     1.133 &     1.031 &       NaN &       NaN \\
%         & Accuracy &    0.803 &       NaN &     0.710 &     0.746 &       NaN &       NaN \\
%     113 & Arousal\_CCC &    0.609 &       NaN &     0.564 &       NaN &     0.605 &       NaN \\
%         & Valence\_CCC &    0.840 &       NaN &     0.805 &       NaN &     0.807 &       NaN \\
%         & nLoss &    0.870 &       NaN &     1.143 &       NaN &     1.011 &       NaN \\
%         & Accuracy &    0.802 &       NaN &     0.708 &       NaN &     0.757 &       NaN \\
%     \bottomrule
%     \end{tabular}
%     \caption{Mixup}
%     \label{tab:my_label}
% \end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|cc}
%     \toprule
%                       &     &  50-60 &  60-85 \\
%     \midrule
%     \hhline{====}
%     w\backslash o       & Ar   & - &  0.529 \\
%     \textrm{60-85}      & Val  & - &  0.789 \\
%                         & Loss & - &    1.2 \\
%                         & Acc  & - &  0.695 \\\hline
%     w\backslash o       & Ar   &  0.573 &      - \\
%     \textrm{50-60}      & Val  &  0.817 &      - \\
%                         & Loss &   1.12 &      - \\
%                         & Acc  &  0.716 &      - \\\hline
%     w\backslash o       & Ar   &  0.565 &  0.496 \\
%     \textrm{50-60}      & Val  &  0.816 &  0.772 \\
%     \textrm{\&60-85}    & Loss &   1.11 &   1.28 \\
%                         & Acc &  0.709 &  0.675 \\\hline
%     \bottomrule
%     \end{tabular}
%     \caption{CDANN 0-1-101 train}
%     \label{tab:cdann_0_1_101_train}
% \end{table}

% \begin{table*}[t]
%     \centering
    
%     \begin{tabular}{ cccc }   % top level tables, with 2 columns
%     (A) & (B) & (C) & (D)\\  
% % leftmost table of the top level table
% \begin{tabular}{c@{\hspace{1.15\tabcolsep}}|c@{\hspace{1.15\tabcolsep}}|c@{\hspace{1.15\tabcolsep}}c@{\hspace{1.15\tabcolsep}}}
%             \toprule
%                               &     &  40-50 &  60-85 \\
%             \midrule
%             \hhline{====}
%             Without       & Ar   &      - &  0.53 \\
%             \textrm{60-85}      & Val  &      - &  0.79 \\
%                                 & Loss &      - &    1.2 \\
%                                 & Acc  &      - &  0.70 \\\hline
%             Without       & Ar   &  0.62 &      - \\
%             \textrm{40-50}      & Val  &  0.83 &      - \\
%                                 & Loss &  0.98 &      - \\
%                                 & Acc  &  0.75 &      - \\\hline
%             Without       & Ar   &  0.59 &  0.49 \\
%             \textrm{40-50}      & Val  &  0.82 &  0.77 \\
%             \textrm{\&60-85}    & Loss &    1.1 &   1.39 \\
%                                 & Acc &  0.74 &  0.66 \\\hline
%             \bottomrule
%             \end{tabular} &  % starting rightmost sub table
% % table 2
% \begin{tabular}{c@{\hspace{1.15\tabcolsep}}|c@{\hspace{1.15\tabcolsep}}c@{\hspace{1.15\tabcolsep}}}
%             \toprule
%                               &       30-40 &  60-85 \\
%             \midrule
%             \hhline{===}
%             Without       &      - &  0.53 \\
%             \textrm{60-85}      &      - &  0.79 \\
%                                 &      - &    1.2 \\
%                                 &      - &  0.70 \\\hline
%             Without       &   0.62 &      - \\
%             \textrm{30-40}      &  0.82 &      - \\
%                                 &  0.95 &      - \\
%                                 &  0.77 &      - \\\hline
%             Without       &  0.60 &  0.49 \\
%             \textrm{30-40}      &  0.82 &  0.79 \\
%             \textrm{\&60-85}    &  0.99 &   1.29 \\
%                                 &  0.76 &  0.68 \\\hline
%             \bottomrule
%             \end{tabular} &
% \begin{tabular}{c@{\hspace{1.15\tabcolsep}}|c@{\hspace{1.15\tabcolsep}}c@{\hspace{1.15\tabcolsep}}}
%     \toprule
%                       &       40-50 &  50-60 \\
%     \midrule
%     \hhline{===}
%     Without       &      - &  0.57 \\
%     \textrm{50-60}      &      - &  0.82 \\
%                         &      - &   1.12 \\
%                         &      - &  0.72 \\\hline
%     Without       &  0.62 &      - \\
%     \textrm{40-50}      &  0.83 &      - \\
%                         &  0.98 &      - \\
%                         &  0.75 &      - \\\hline
%     Without       &  0.60 &  0.56 \\
%     \textrm{40-50}      &  0.82 &  0.81 \\
%     \textrm{\&50-60}    &   1.03 &   1.15 \\
%                         &  0.75 &   0.71 \\\hline
%     \bottomrule
%     \end{tabular} &

%     \begin{tabular}{c@{\hspace{1.15\tabcolsep}}|c@{\hspace{1.15\tabcolsep}}c@{\hspace{1.15\tabcolsep}}}
%     \toprule
%                       &       30-40 &  50-60 \\
%     \midrule
%     \hhline{===}
%     Without       &      - &  0.57 \\
%     \textrm{50-60}      &      - &  0.82 \\
%                         &      - &   1.12 \\
%                         &      - &  0.72 \\\hline
%     Without       &   0.62 &      - \\
%     \textrm{30-40}      &  0.82 &      - \\
%                         &  0.95 &      - \\
%                         &  0.77 &      - \\\hline
%     Without       &  0.60 &  0.54 \\
%     \textrm{30-40}      &  0.81 &  0.80 \\
%     \textrm{\&50-60}    &   1.09 &   1.33 \\
%                         &  0.75 &  0.70 \\\hline
%     \bottomrule
%     \end{tabular}   
    
% \end{tabular}

%     \caption{Performance on unseen domains' training sets.}
%     \label{tab:unseen_train_domains}
% \end{table*}


% \begin{figure}[]
%     \centering
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \begin{table}[]
%             \centering
%             \begin{tabular}{c|c|cc}
%             \hhline{====}
%             \toprule
%                               &     &  40-50 &  60-85 \\
%             \midrule
%             \hline
%             w\backslash o       & Ar   &      - &  0.529 \\
%             \textrm{60-85}      & Val  &      - &  0.789 \\
%                                 & Loss &      - &    1.2 \\
%                                 & Acc  &      - &  0.695 \\\hline
%             w\backslash o       & Ar   &  0.615 &      - \\
%             \textrm{40-50}      & Val  &  0.826 &      - \\
%                                 & Loss &  0.983 &      - \\
%                                 & Acc  &  0.751 &      - \\\hline
%             w\backslash o       & Ar   &  0.589 &  0.491 \\
%             \textrm{40-50}      & Val  &  0.818 &  0.765 \\
%             \textrm{\&60-85}    & Loss &    1.1 &   1.39 \\
%                                 & Acc &  0.735 &  0.664 \\\hline
%             \bottomrule
%             \end{tabular}
%             \caption{CDANN 0-2-102 train}
%             \label{tab:cdann_0_2_102_train}
%         \end{table}
%     \end{minipage}%
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         \begin{table}[]
%             \centering
%             \begin{tabular}{c|c|cc}
%             \toprule
%                               &     &  30-40 &  60-85 \\
%             \midrule
%             \hhline{====}
%             w\backslash o       & Ar   &      - &  0.529 \\
%             \textrm{60-85}      & Val  &      - &  0.789 \\
%                                 & Loss &      - &    1.2 \\
%                                 & Acc  &      - &  0.695 \\\hline
%             w\backslash o       & Ar   &   0.62 &      - \\
%             \textrm{30-40}      & Val  &  0.823 &      - \\
%                                 & Loss &  0.947 &      - \\
%                                 & Acc  &  0.767 &      - \\\hline
%             w\backslash o       & Ar   &  0.601 &  0.491 \\
%             \textrm{30-40}      & Val  &  0.821 &  0.787 \\
%             \textrm{\&60-85}    & Loss &  0.991 &   1.29 \\
%                                 & Acc  &  0.756 &  0.679 \\\hline
%             \bottomrule
%             \end{tabular}
%             \caption{CDANN 0-3-103 train}
%             \label{tab:cdann_0_3_103_train}
%         \end{table}
%     \end{minipage}
% \end{figure}





% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|cc}
%     \toprule
%                       &     &  40-50 &  50-60 \\
%     \midrule
%     \hhline{====}
%     w\backslash o       & Ar   &      - &  0.573 \\
%     \textrm{50-60}      & Val  &      - &  0.817 \\
%                         & Loss &      - &   1.12 \\
%                         & Acc  &      - &  0.716 \\\hline
%     w\backslash o       & Ar   &  0.615 &      - \\
%     \textrm{40-50}      & Val  &  0.826 &      - \\
%                         & Loss &  0.983 &      - \\
%                         & Acc  &  0.751 &      - \\\hline
%     w\backslash o       & Ar   &  0.604 &  0.563 \\
%     \textrm{40-50}      & Val  &  0.823 &  0.813 \\
%     \textrm{\&50-60}    & Loss &   1.03 &   1.15 \\
%                         & Acc  &  0.746 &   0.71 \\\hline
%     \bottomrule
%     \end{tabular}
%     \caption{CDANN 1-2-112 train}
%     \label{tab:cdann_1_2_112_train}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|cc}
%     \toprule
%                       &     &  30-40 &  50-60 \\
%     \midrule
%     \hhline{====}
%     w\backslash o       & Ar   &      - &  0.573 \\
%     \textrm{50-60}      & Val  &      - &  0.817 \\
%                         & Loss &      - &   1.12 \\
%                         & Acc  &      - &  0.716 \\\hline
%     w\backslash o       & Ar   &   0.62 &      - \\
%     \textrm{30-40}      & Val  &  0.823 &      - \\
%                         & Loss &  0.947 &      - \\
%                         & Acc  &  0.767 &      - \\\hline
%     w\backslash o       & Ar   &  0.596 &  0.541 \\
%     \textrm{30-40}      & Val  &  0.812 &  0.803 \\
%     \textrm{\&50-60}    & Loss &   1.09 &   1.33 \\
%                         & Acc  &  0.753 &  0.695 \\\hline
%     \bottomrule
%     \end{tabular}
%     \caption{CDANN 1-3-113 train}
%     \label{tab:cdann_1_3_113_train}
% \end{table}
